Beyond Single-Model Views for Deep Learning: Optimization versus Generalizability of Stochastic Optimization Algorithms

Despite an extensive body of literature on deep learning optimization, our current understanding of what makes an optimization algorithm effective is fragmented. In particular, we do not understand well whether enhanced optimization translates to improved generalizability. Current research overlooks the inherent stochastic nature of stochastic gradient descent (SGD) and its variants, resulting in a lack of comprehensive benchmarking and insight into their statistical performance. This paper aims to address this gap by adopting a novel approach. Rather than solely evaluating the endpoint of individual optimization trajectories, we draw from an ensemble of trajectories to estimate the stationary distribution of stochastic optimizers. Our investigation encompasses a wide array of techniques, including SGD and its variants, flat-minima optimizers, and new algorithms we propose under the Basin Hopping framework. Through our evaluation, which encompasses synthetic functions with known minima and real-world problems in computer vision and natural language processing, we emphasize fair benchmarking under a statistical framework, comparing stationary distributions and establishing statistical significance. Our study uncovers several key findings regarding the relationship between training loss and hold-out accuracy, as well as the comparable performance of SGD, noise-enabled variants, and novel optimizers utilizing the BH framework. Notably, these algorithms demonstrate performance on par with flat-minima optimizers like SAM, albeit with half the gradient evaluations. We anticipate that our work will catalyze further exploration in deep learning optimization, encouraging a shift away from single-model approaches towards methodologies that acknowledge and leverage the stochastic nature of optimizers.

==> TODO/Box-plots.tex <==
We owe box plots in the Supplementary Material.

I want to add four sets of plots. 

Set 1: show loss of SetA (the 50 lowest-loss models)

Four box plots, one per each real-world task. The algorithms (named as in paper, no adaptive included) are on the x axis. Loss is on the y axis.


Set 2: show loss of SetB (the 50 highest accuracy/F1 models)

Four box plots, one per each real-world task. The algorithms (named as in paper, no adaptive included) are on the x axis. Loss is on the y axis.


Set 3: show accuracy/F1 of SetA (the 50 lowest-loss models)

Four box plots, one per each real-world task. The algorithms (named as in paper, no adaptive included) are on the x axis. Accuracy/F1 is on the y axis.


Set 4: show accuracy/F1 of SetB (the 50 highest accuracy/F1 models)

Four box plots, one per each real-world task. The algorithms (named as in paper, no adaptive included) are on the x axis. Accuracy/F1 is on the y axis.



==> TODO/Code-In-Github.tex <==
Self explanatory.
Work with Sam.

Only put code as of what you submitted today.

The additions to the supplementary material (other to-dos listed here) do not have to be added to the code in github.

==> TODO/More-Synthetic-Functions.tex <==
More synthetic functions over the three we show in the paper. Please add to both results and the exposition in the Supplementary 
Material that shows countour plots and lists the minima:

(4)
Rosenbrock function -- https://www.sfu.ca/~ssurjano/rosen.html
The Rosenbrock function is a non-convex function.The global minimum is inside a long, narrow, parabolic shaped flat valley. To find the valley is trivial. To converge to the global minimum, however, is difficult.

(5)
Beale function -- https://www.sfu.ca/~ssurjano/beale.html
The Beale function has one global minimum but a very broad plateau where optimization algorithms can get stuck (and many shallow local minima). We can evaluate simply \% in global minimum versus else. The domain is given in the above link.

(6)
Goldstein–Price function -- https://www.sfu.ca/~ssurjano/goldpr.html
The Goldstein–Price function has one global minimum and several local minima. The domain is given in the link.
This link, https://rdrr.io/cran/DiceOptim/src/R/goldsteinprice.R, uses a standardized version with one global minimum and three local minima.


- The local minima : 

$(-1.84775, 0.07743) $ with a value of $-3.36177$
$(-0.85031, -1.37621)$ with a value of $-3.43107$
$(1.06449, -0.62385)$ with a value of $-3.33839$
$(0.56231, 2.30603)$ with a value of $-3.42786$
$(-0.96171, 2.37411)$ with a value of $-3.38648$



(7)
Cross-in-tray function -- https://www.sfu.ca/~ssurjano/crossit.html
The Cross-in-Tray function has multiple (4) global minima. It has a characteristic 'cross.' We can evaluate \% of each of the global minima versus else. The domain is given in the link.
-The global minimas : 
(1, 1) with a value of 0
(-1, 1) with a value of 16
(1, -1) with a value of 16
(-1, -1) with a value of 36
(8)
Bukin function N.6 -- https://www.sfu.ca/~ssurjano/bukin6.html
The sixth Bukin function has many local minima, all of which lie in a ridge. Difficult to optimize. We will evaluate just \% in global minimum versus else. The domain is given in the link.


- How can we plot this? Global vs others? 

(9)
Eggholder function -- https://www.sfu.ca/~ssurjano/egg.html
The Eggholder function is a difficult function to optimize, because of the large number of local minima. We will evaluate just \% in global minimum versus else. The domain is given in the link.

(10)
Rastrigin function -- https://www.sfu.ca/~ssurjano/rastr.html
The Rastrigin function has several local minima that are regularly distributed. It is a good example of a non-convex optimization algorithm getting stuck. We can measure the \% of times in global minimum versus else. The domain is given in the link.

(11)

DIXON-PRICE FUNCTION

https://www.sfu.ca/~ssurjano/dixonpr.html

For 2 dimensions, the Dixon-Price function has two local minimas. They are located at the points (1, 0) and (0, 1). 
The global minimum of the Dixon-Price function is located at the point (1, 1). However, the function is non-convex, so it can have many local minima


==> TODO/MoreLearningCurves.tex <==
Do the learning curves for the other two tasks, as well

==> TODO/MorepairwiseComparisons.tex <==
Compare SGD to NiG-SGD
Compare SGD to NiM-SGD

Compare SAM to NiG-SGD
Compare SAM to NiM-SGD

Compare SGD to NiG-BH
Compare SGD to NiM-BH (you have done)

Compare SGD to NiG-MpBH
Compare SGD to NiM-MpBH

Compare SAM to NiG-BH
Compare SAM to NiM-BH (you have done)

Compare SAM to NiG-MpBH
Compare SAM to NiM-MpBH

Compare NiG-BH to NiM-BH
Compare NiG-BH to NiG-MpBH
Compare NiG-BH to NiM-MpBH

Compare NiM-BH to NiG-MpBH
Compare NiM-BH to NiM-MpBH



==> TODO/New-BudgetConstrained-Analysis.tex <==
Restrict budget of SAM to that of the others. Call this SAMc (c for constrained).

Extract its SetA and SetB in this constrained budget. 
Add new row in Table 3, SamC, right below SAM. Report on tasks as you have done in Table 3.


==> TODO/RealWorld_Problems.tex <==
Imagenet on ResNet 50 (Running)

Training can be using Pre-Trained Imagenet weights and then running for multiple epochs 
Current one is running from scratch

https://github.com/Lornatang/ResNet-PyTorch

COCO/KITTI dataset- Object detection 

Machine Translation?????? - Generative models




Should we pursue this? Or at least some of them?: 


The GLUE benchmark tasks include:

\textbf{CoLA:} The Corpus of Linguistic Acceptability task measures the ability of a model to determine whether a sentence is grammatically correct.

\textbf{SST-2:} The Stanford Sentiment Treebank task measures the ability of a model to determine the sentiment of a sentence, i.e., whether it is positive, negative, or neutral.

\textbf{MRPC:} The Microsoft Research Paraphrase Corpus task measures the ability of a model to determine whether two sentences are paraphrases of each other.

\textbf{STS-B: }The Semantic Textual Similarity Benchmark task measures the ability of a model to determine the similarity of two sentences.

\textbf{QQP:} The Quora Question Pairs task measures the ability of a model to determine whether two questions are semantically equivalent.

\textbf{MNLI:} The MultiNLI (Multi-Genre Natural Language Inference) task measures the ability of a model to determine the entailment relationship between two sentences.
RTE: The Recognizing Textual Entailment task measures the ability of a model to determine whether one sentence entails another sentence.

\textbf{WNLI:} The Winograd Schema Challenge task measures the ability of a model to correctly resolve pronoun references in a sentence.

\textbf{Diagnostic:} A diagnostic dataset used to evaluate a model's performance on a wide range of linguistic phenomena.



==> TODO/Statistical-Tests.tex <==
In the main paper we compared the accuracy/F1 of SetA to the accuracy/F1 of Set B.

Let us please also compare the loss of SetA to the loss of SetB. Do only on tuned algorithms (no base needed). Both Mann Whitney U and t-tests. Result: two tables.

Question/null hypothesis we are exploring now is: are the best performing models (on accuracy/F1)/SetB the same in loss as the ones selected by loss (SetA)

==> copyright.tex <==
\section{Copyright}
All papers submitted for publication by AAAI Press must be accompanied by a valid signed copyright form. They must also contain the AAAI copyright notice at the bottom of the first page of the paper. There are no exceptions to these requirements. If you fail to provide us with a signed copyright form or disable the copyright notice, we will be unable to publish your paper. There are \textbf{no exceptions} to this policy. You will find a PDF version of the AAAI copyright form in the AAAI AuthorKit. Please see the specific instructions for your conference for submission details.

==> sections/Acknowledgements.tex <==
\section{Acknowledgements}
\label{sec:Acknowledgements}

We are grateful to Arindam Banerjee and Sanmi Koyejo for initial discussions on this work. Computations were run on the Hopper, a research computing cluster provided by the Office of Research Computing at George Mason University. 

==> sections/oldFunctionExposition.tex <==
\begin{table}[htbp]
\centering
\tiny
\begin{tabular}{|p{5em}||p{2em}|p{2em}|p{2em}|p{2em}|p{2em}|}
\hline
\textbf{Algorithm} & \textbf{GM1} & \textbf{GM2} & \textbf{GM3} & \textbf{GM4} & \textbf{Else}\\
\hline
GD &  28 &  25 & 23 &  24 & 0\\

NiG-GD & 28 & 23 & 23 & 25 & 1\\

NiM-GD & 30 & 27 & 23 & 20 & 0\\

SAM &  30 &  23 & 20 & 20 & 7\\

NiG-BH & 27 & 25 & 25 & 22 & 1\\

NiM-BH &  27 & 25 & 24 & 24 & 0\\

NiG-MBH & 22 & 27 & 23 & 28 & 0\\

NiM-MBH & 30 & 23 & 20 & 20 & 7\\

NiG-MpBH & 25 & 28 & 21 & 25 & 1\\

NiM-MpBH & 28 & 25 & 23 & 23 & 1\\

%NiG-AdBH & 26 & 25 & 22 & 22 & 5\\

%NiM-AdBH & 28 & 27 & 23 & 22 & 0\\
\hline
\end{tabular}
\vspace*{-2mm}\caption{\small The stationary distribution (reported in \% for each entry) for the Himmelblau function for each algorithm. The function has four global minima, as listed in the Supplementary Material.}
\label{table:SyntheticFunctions-StationaryDistribution-Comparison-Himmelblau}
\end{table}


%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%% Three-Hump Camel

\begin{table}[htbp]
\centering
\tiny
\begin{tabular}{|p{5em}||p{2em}|p{2em}|p{2em}|p{2em}|}
\hline
\textbf{Algorithm} & \textbf{GM} & \textbf{LM1} & \textbf{LM2} & \textbf{Else}\\
\hline
GD & 32 & 35 & 33 & 0\\

NiG-GD & 31 & 35 & 34 & 0\\

NiM-GD & 34 & 34 & 32 & 0\\

SAM & 30 & 27 & 25 & 18 \\

NiG-BH & 32 & 35 & 33 & 0\\

NiM-BH & 33 & 35 & 31 & 1\\

NiG-MBH & 33 & 33 & 34 & 0\\

NiM-MBH & 34 & 32 & 34 & 0\\

NiG-MpBH & 30 & 35 & 35 & 5\\

NiM-MpBH & 32 & 36 & 32 & 0\\

%NiG-AdBH & 34 & 32 & 34 & 0\\

%NiM-AdBH & 33 & 33 & 34 & 0\\
\hline
\end{tabular}
\vspace*{-2mm}\caption{\small The stationary distribution (reported in \% for each entry) for the Three-Hump Camel function for each algorithm. The function has one global minimum and two local minima, as listed in the Supplementary Material.}
\label{table:SyntheticFunctions-StationaryDistribution-Comparison-Three-Hump-Camel}
\end{table}



%%%%%%%%%%%%%%%%%%
%%%Six-Hump Camel

\begin{table}[htbp]
\centering
\tiny
\begin{tabular}{|p{5em}||p{2em}|p{2em}|p{2em}|p{2em}|p{2em}|p{2em}|p{2em}|}
\hline
\textbf{Algo} & \textbf{GM1} & \textbf{GM1} & \textbf{LM1} & \textbf{LM2} &\textbf{LM3} & \textbf{LM4} & \textbf{Else}\\
\hline
GD &  4.25 &  23.5  &  22.75 & 17.25 &  1.5 &  10.25 & 20.5 \\

NiG-GD & 13.5  &	16.4  &	14.6  &  	15.5 &	0.4  &	1.6 & 38 \\

NiM-GD & 7.375  &	18.38 	& 19.88  &	16.5 	& 10   &	9.86 &	17 \\

SAM & 11.63 &16. 1 &	19  &	16.13 &	0.75 &	3 & 34  \\

NiG-BH & 6.25 & 21.75 & 21.75 & 17.75 &   2.   &  8.25 & 22\\

NiM-BH & 6.5 & 20.25 & 21.75 & 17.25&   2.25 & 10.25 & 22\\

NiG-MBH & 5.75 &  23.75 & 24.25 & 16.25  & 2 & 11 & 17\\

NiM-MBH & 5.25 & 24.75 & 24.25 & 16.5 &    1.75 & 11.5 & 12\\

NiG-MpBH & 5.75 & 23.75 & 24.5 & 17.25  & 1.15  & 11.25 & 16.3\\

NiM-MpBH & 6  & 22  &   22.75  & 16  &    2 &     9 & 22 \\

%NiG-AdBH & 26\% & 32\% & 28\% & 14\%\\

%NiM-AdBH & 28\% & 27\% & 34\% & 11\%\\
\hline
\end{tabular}
\vspace*{-2mm}\caption{\small The stationary distribution (reported in \% for each entry) for the Six-Hump Camel function for each algorithm. The function has two global minima and two local minima, as listed in the Supplementary Material.}
\label{table:SyntheticFunctions-StationaryDistribution-Comparison-Six-Hump-Camel}
\end{table}

